Rapid Neural Architecture Search by Learning to Generate Graphs from Datasets

Despite the success of recent Neural Architecture Search (NAS) methods on various tasks which have shown to output networks that largely outperform human-designed networks, conventional NAS methods have mostly tackled the optimization of searching for the network architecture for a single task (dataset), which does not generalize well across multiple tasks (datasets). Moreover, since such task-specific methods search for a neural architecture from scratch for every given task, they incur a large computational cost, which is problematic when the time and monetary budget are limited. In this paper, we propose an efficient NAS framework that is trained once on a database consisting of datasets and pretrained networks and can rapidly search for a neural architecture for a novel dataset. The proposed MetaD2A (Meta Dataset-to-Architecture) model can stochastically generate graphs (architectures) from a given set (dataset) via a cross-modal latent space learned with amortized meta-learning. Moreover, we also propose a meta-performance predictor to estimate and select the best architecture without direct training on target datasets. The experimental results demonstrate that our model meta-learned on subsets of ImageNet-1K and architectures from NAS-Bench 201 search space successfully generalizes to multiple unseen datasets including CIFAR-10 and CIFAR-100, with an average search time of 33 GPU seconds. Even under MobileNetV3 search space, MetaD2A is 5.5K times faster than NSGANetV2, a transferable NAS method, with comparable performance. We believe that the MetaD2A proposes a new research direction for rapid NAS as well as ways to utilize the knowledge from rich databases of datasets and architectures accumulated over the past years. Code is available at https://github.com/HayeonLee/MetaD2A.

==> others/algorithms.tex <==
\begin{minipage}{.52\linewidth}
%\vspace{-0.01in}

\begin{algorithm}[H]
	\caption{Meta-training}\label{algo:algorithm1}
	\small
	\begin{algorithmic}[1]
		\State \textbf{Input:} $(\D^{1},\tilde{\G}^{1}),\dots,(\D^{N_{mtr}},\tilde{\G}^{N_{mtr}})$
		\State \textbf{Input:} Pretrained $\theta$, Learning rate $\alpha_{\phi}$, $\alpha_{\theta}$
		\State \textbf{Output:} $\phi^*$, $\theta^*$
		\State Randomly initialize $\phi$
		\While{not converged}
% 		\State $\mathcal{L}^\te \leftarrow 0$
		\For{$\tau=1$ to $N_{mtr}$}
		\State Randomly sample $\mathcal{B}^\tau \subset \D^\tau$
		\State Compute $\G^\tau = Dec_{\bm{\theta}} \big( Enc_{\bm{\phi}} \big( \mathcal{B}^\tau \big)\big)$
		\State Compute $\mathcal{L}^\tau_{\bm{\phi}, \bm{\theta}}(\D^\tau, \tilde{\G}^\tau)$
		\EndFor
		\State $\bm{\phi} \leftarrow \bm{\phi} - \alpha \grad_{\phi} \frac{1}{N_\tau}\sum_{\tau=1}^{N_\tau} \mathcal{L}^\tau_{\bm{\phi}, \bm{\theta}}(\D^\tau,\G^\tau)$
		\State $\bm{\theta} \leftarrow \bm{\theta} - \alpha \grad_{\theta} \frac{1}{N_\tau}\sum_{\tau=1}^{N_\tau} \mathcal{L}^\tau_{\bm{\phi}, \bm{\theta}}(\D^\tau,\G^\tau)$
		\EndWhile
	\end{algorithmic}
	\end{algorithm}
% \vspace{2mm}
\end{minipage}
\begin{minipage}{.48\linewidth}
\begin{algorithm}[H]
	\caption{Meta-test}\label{algo:algorithm2}
	\small
	\begin{algorithmic}[1]
		\State \textbf{Input:} $\hat{\D}^1, ... , \hat{\D}^{N_{mte}}$
		\State \textbf{Input:} $\phi^*$, $\theta^*$
		\State \textbf{Output:} $\G^*$
		\State
		\For{$\tau=1$ to $N_{te}$}
		    \State Randomly sample ${\mathcal{\hat{B}}^\tau} \subset \hat{\D}^{\tau}_{tr}$
		    \State Compute $\G^* = Dec_{\bm{\theta}^*}(Enc_{\bm{\phi}*}({\mathcal{\hat{B}^\tau}}))$ 
		\State Training $\G^*$ on $\hat{\D}^{\tau}_{tr}$ with parameters $\bm{\pi}$
		\State Evaluate $\G^*_{\bm{\pi}^*}$ on $\hat{\D}^{\tau}_{te}$
		\EndFor
		\State
		\State
		\State
	\end{algorithmic}
	\end{algorithm}
% \vspace{2mm}
\end{minipage}


==> others/figure_abl.tex <==
\begin{minipage}[h!]{\textwidth}
	\begin{minipage}{0.68\textwidth}
	    \captionsetup{type=figure} 
		\vspace{-0.1in}
		\centering
    	\subcaptionbox{epoch}
		{\includegraphics[width=.32\linewidth]{figures/3_1.latent_z.png}\label{fig:mimg_tsne}}
		\subcaptionbox{# of input x}
        {\includegraphics[width=.32\linewidth]{figures/3_1.latent_z.png}\label{fig:multi_tsne}}
		\subcaptionbox{Src. D. size}
        {\includegraphics[width=.32\linewidth]{figures/3_1.latent_z.png}\label{fig:multi_tsne}}
		\vspace{-0.1in}
		\captionof{figure}{\small xx.}
		\label{fig:ood}
	\end{minipage}
	%\vspace{0.08in}
	\begin{minipage}{0.31\textwidth}
	    %\vspace{-0.1in}
		\centering 
		\small
		\resizebox{1\textwidth}{!}{
		\begin{tabular}{ccc}
			\hline
			Src. D. & \multicolumn{2}{c}{Accuracy}   
			\\
			Size 
			& CIFAR10 
			& CIFAR100
			\\
			\hline
			100
			& xx.xx\tiny$\pm$x.xx
			& xx.xx\tiny$\pm$x.xx
			\\
			200
			& xx.xx\tiny$\pm$x.xx
			& xx.xx\tiny$\pm$x.xx
			\\
		    300
			& xx.xx\tiny$\pm$x.xx
			& xx.xx\tiny$\pm$x.xx
			\\
			447
			& xx.xx\tiny$\pm$x.xx
			& xx.xx\tiny$\pm$x.xx
			\\
			\hline
		\end{tabular}
		}
	\vspace{0.18in}
	\captionof{table}{\small xx.}\label{tbl:ood}
	\end{minipage}
	\vspace{-0.05in}
\end{minipage}

==> others/figure_bins.tex <==
\begin{figure}[t]
\begin{subfigure}{.5\textwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{figures/3_4.LVRS.png}  
  \caption{OURS-RS}
  \label{fig:sub-first}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{figures/3_4.OURS.png}  
  \caption{OURS}
  \label{fig:sub-second}
\end{subfigure}
\vspace{-0.1in}
\caption{}   
\label{fig:temp}
\vspace{-0.3in}
\end{figure}

==> others/figure_comparision.tex <==
% \begin{figure}[t]
% \begin{subfigure}{.28\textwidth}
%   \centering
%   % include first image
%   \includegraphics[width=\linewidth]{figures/1_concept_1_2.pdf}  
%   \caption{Task-specific NAS}
%   \label{fig:sub-first}
% \end{subfigure}
% \begin{subfigure}{.33\textwidth}
%   \centering
%   % include second image
%   \includegraphics[width=\linewidth]{figures/1_concept_2.pdf}  
%   \caption{Meta-NAS}
%   \label{fig:sub-second}
% \end{subfigure}
% \begin{subfigure}{.40\textwidth}
%   \centering
%   % include first image
%   \includegraphics[width=\linewidth]{figures/1_concept_3.pdf}  
%   \caption{MetaD2A (Ours)}
%   \label{fig:sub-third}
% \end{subfigure}
% \vspace{-0.1in}
% \caption{\small \textbf{Comparison of our method to existing NAS approaches} \textbf{(a)} Task-specific NAS methods require large search time as the search needs to be done from scratch for each task $\tau_i$. \textbf{(b)} Meta-NAS methods can rapidly adapt to new tasks by leveraging meta-knowledge, but they do not scale well to large datasets and networks due to inefficiency in the meta-learning framework. \textbf{(c)} Our method can instantly generate a task-specific architecture for a given dataset with amortized meta-learning of the cross-modal latent space with the set encoder and the graph decoder. } 
% \label{fig:comparison_NAS}
% \vspace{-0.2in}
% \end{figure}

\begin{figure}[t]
\begin{subfigure}{.258\textwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{figures/1_concept_1_4.pdf}  
  \caption{Task-specific NAS}
  \label{fig:sub-first}
\end{subfigure}
\begin{subfigure}{.325\textwidth}
  \centering
%   % include second image
  \includegraphics[width=\linewidth]{figures/1_concept_2_4.pdf}  
   \caption{Meta-NAS}
   \label{fig:sub-second}
 \end{subfigure}
 \begin{subfigure}{.405\textwidth}
   \centering
%   % include first image
   \includegraphics[width=\linewidth]{figures/1_concept_3_4.pdf}  
   \caption{MetaD2A (Ours)}
   \label{fig:sub-third}
 \end{subfigure}
 \vspace{-0.1in}
\caption{\small \textbf{Comparison of our method to conventional NAS approaches} \textbf{(a)} Task-specific NAS methods require enormous search time as the search needs to be done from scratch for each task. \textbf{(b)} Meta-NAS methods can adapt to new tasks by leveraging meta-knowledge, but they do not scale well to large datasets and networks due to inefficiency in the meta-learning framework. \textbf{(c)} Our method can rapidly generate set-specific neural architecture candidates for a given dataset with amortized meta-learning of the cross-modal latent space which maps the dataset to architecture, with the set encoder and the graph decoder. Then, our performance predictor selects the best architecture among the generated architectures based on predicted performance.} 
\label{fig:comparison_NAS}
\vspace{-0.2in}
\end{figure}

==> others/figure_concept.tex <==
\begin{figure}[t]
\centering
% \includegraphics[width=\linewidth]{figures/2_overall_architecture_5.pdf}  
\begin{subfigure}{.855\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures/2_overall_architecture_10.pdf}  
  %\vspace{-0.2in}
  \caption{}%\small Overview of MetaD2A}
\end{subfigure}
\begin{subfigure}{.135\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures/2_overall_architecture_8_metric.pdf}  
 % \vspace{+0.1in}
  \caption{}%\small T-SNE vis. of Latent Space }
\end{subfigure}
\vspace{-0.1in}
\caption{\small \textbf{(a) Overview of MetaD2A} 
MetaD2A generator with $\bm{\theta}$ and $\bm{\phi}$ meta-learns the set-dependent DAGs representations on the training tasks, which are the subset of ImageNet-1K. MetaD2A predictor with $\bm{\omega}$ meta-learns to predict performance across the multiple tasks. We transfer MetaD2A to new target datasets to search for the set-specific architecture within a minute. \textbf{(b)} T-SNE visualization of a learned cross-modal latent space. }% The closest to the given dataset the architecture embedding is, the better performance is obtained on the given dataset than the farthest.}
\label{fig:concept}
\vspace{-0.15in}
\end{figure}

==> others/figure_graph_decoder.tex <==


\begin{wrapfigure}{t}{0.3\linewidth}
  %\vspace{-0.2in}
  \centering
  \includegraphics[width=\linewidth]{figures/2_graph_decoder.pdf}  
  \vspace{-0.25in}
  \caption{\small Graph Decoder} \label{fig:graph_decoder}
\vspace{-0.15in}
\end{wrapfigure}


==> others/figure_graph_encoder.tex <==


\begin{wrapfigure}{t}{0.33\linewidth}
  \vspace{-0.2in}
  \centering
  \includegraphics[width=\linewidth]{figures/2_graph_encoder.pdf}  
  \vspace{-0.25in}
  \caption{\small Bi-dir. Encoding} \label{fig:graph_encoder}
\vspace{-0.15in}
\end{wrapfigure}


==> others/figure_hier_setpooling.tex <==


\begin{wrapfigure}{t}{0.22\linewidth}
  \vspace{-0.2in}
  \centering
  \includegraphics[width=\linewidth]{figures/2_hier_set_pooling.pdf}  
  \vspace{-0.3in}
  \caption{\small Set Encoder} \label{fig:hier_set_pooling}
\vspace{-0.15in}
\end{wrapfigure}


==> others/figure_hist_time_acc.tex <==
\begin{minipage}[t!]{\linewidth}
	\centering
	\begin{minipage}{0.49\linewidth}
	    \captionsetup{type=figure} 
		\vspace{-0.1in}
		\centering
            \subcaptionbox{}
            {\includegraphics[width=.48\linewidth]{figures/3_3.time_acc.png}}
            \subcaptionbox{}
            {\includegraphics[width=.48\linewidth]{figures/3_3.param_acc.png}}
        \setcounter{figure}{2}
        \vspace{-0.1in}
		\captionof{figure}{\small \textbf{(a) Time vs. Acc. (b) Params. vs. Acc.}}
    	\label{fig:time_params_acc}
	\end{minipage}
	\begin{minipage}{0.49\linewidth}
		\captionsetup{type=figure} 
		\vspace{-0.1in}
		\centering
		 \subcaptionbox{\small Ours-RS}
         {\includegraphics[width=.49\linewidth]{figures/3_4.OURS-RS.png}}
         \subcaptionbox{\small Ours}
         {\includegraphics[width=.49\linewidth]{figures/3_4.OURS.png}}
		\setcounter{figure}{3}
        \vspace{-0.1in}
		\captionof{figure}{\small \textbf{Acc. distribution of 20 MetaD2A tasks.}}
		\label{fig:acc_dist}
	\end{minipage}
\end{minipage}


==> others/figure_hist_time_acc2.tex <==
% \begin{wrapfigure}{t}{0.45\linewidth}
% 	\centering
% 	\vspace{-0.2in}
% \begin{subfigure}{.49\linewidth}
%   \vspace{-0.05in}
%   \centering
%   \includegraphics[width=\linewidth]{figures/3_3.time_acc.png}  
%   \label{fig:time_acc}
%   \vspace{-0.25in}
%   \end{subfigure}
% \begin{subfigure}{.49\linewidth}
%   \centering
%   \includegraphics[width=\linewidth]{figures/3_4.OURS.png}  
% %   \caption{\small \textbf{Accuracy vs. Parameters}}
% %   \caption{}
% %   \caption{}
%   \label{fig:time_acc}
% 	\vspace{-0.25in}
% \end{subfigure}
% \caption{}
% \vspace{-0.2in}
% \end{wrapfigure}

\begin{wrapfigure}{t}{0.30\linewidth}
  \vspace{-0.2in}
  \centering
  \includegraphics[width=\linewidth]{figures/3_3.time_acc.png}  
  \vspace{-0.25in}
  \caption{ Time vs. Accuracy} \label{fig:time_acc}
\vspace{-0.15in}
\end{wrapfigure}


==> others/figure_model_component.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}{.33\linewidth}
  \centering
  \vspace{-0.1in}
  \includegraphics[width=\linewidth]{figures/2_hier_set_pooling.pdf}  
  \vspace{-0.2in}
  \caption{Hierarchical Set Pooling}
\end{subfigure}
\begin{subfigure}{.3\linewidth}
  \centering
  \vspace{-0.1in}
  \includegraphics[width=\linewidth]{figures/2_graph_decoder.pdf}
  \vspace{-0.2in}
  \caption{GNN-AMP Graph Decoder}
\end{subfigure}
\begin{subfigure}{.355\linewidth}
  \centering
  \vspace{-0.1in}
  \includegraphics[width=\linewidth]{figures/2_graph_encoder.pdf} 
  \vspace{-0.2in}
  \caption{GNN-AMP Graph Encoder}
\end{subfigure}
\vspace{-0.15in}
\caption{\small \textbf{(a)} Hierarchical Set Pooling is the attention-based module to extract a set latent vector for DAG generation considering class label information from $\mathcal{D}$. \textbf{(b)} GNN-AMP Graph Decoder generates the set-dependent DAG from the latent vector with asynchronous message passing. \textbf{(c)} GNN-AMP Graph Encoder for the performance predictor summarizes the input DAG into a single vector with bi-directional encoding scheme.}
\label{fig:model_component}
\vspace{-0.15in}
\end{figure}

==> others/figure_param_acc.tex <==
% \begin{figure}[t]
% \centering
% \includegraphics[width=0.5\linewidth]{figures/3_3.time_acc2.PNG}  
% \caption{Concept of our method}
% \label{fig:time_acc}
% \end{figure}

\begin{wrapfigure}{t}{0.45\linewidth}
	\centering
	\vspace{-0.2in}
\begin{subfigure}{.49\linewidth}
  \vspace{-0.05in}
  \centering
  \includegraphics[width=\linewidth]{figures/3_3.time_acc.png}  
%   \caption{\small \textbf{Accuracy vs. Search Time}}
%   \caption{}
  \label{fig:time_acc}
  \vspace{-0.25in}
  \end{subfigure}
\begin{subfigure}{.49\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures/3_3.param_acc.png}  
%   \caption{\small \textbf{Accuracy vs. Parameters}}
%   \caption{}
%   \caption{}
  \label{fig:time_acc}
	\vspace{-0.25in}
\end{subfigure}
\caption{}
\vspace{-0.2in}
% 	\includegraphics[width=\linewidth]{figures/3_3.param_acc.png}
% 	\vspace{-0.25in}
% 	\caption{\small \textbf{Accuracy vs. Parameters}}
% 	\label{fig:time_acc}
% 	\vspace{-0.1in}
\end{wrapfigure}

==> others/figure_pp_datasize.tex <==
\begin{wrapfigure}{t}{0.493\linewidth}
  \vspace{-0.2in}
  \centering
	\includegraphics[width=0.4935\linewidth]{figures/5_pp_abl_datasize_CIAFR10.png}
    \includegraphics[width=0.4935\linewidth]{figures/5_pp_abl_datasize_CIAFR100.png}
\vspace{-0.25in}
  \caption{\small Acc. and Corr. over training task size} \label{fig:pp_abl_datasize}
\vspace{-0.15in}
\end{wrapfigure}


==> others/figure_time_acc.tex <==
% \begin{figure}[t]
% \centering
% \includegraphics[width=0.5\linewidth]{figures/3_3.time_acc2.PNG}  
% \caption{Concept of our method}
% \label{fig:time_acc}
% \end{figure}

\begin{wrapfigure}{t}{0.35\linewidth}
	\centering
	\vspace{-0.2in}
	\includegraphics[width=\linewidth]{figures/3_3.time_acc.PNG}
	\vspace{-0.25in}
	\caption{\small \textbf{Accuracy vs. Search Time}}
	\label{fig:time_acc}
	\vspace{-0.1in}
\end{wrapfigure}

==> others/figure_vis.tex <==
% \setcounter{figure}{3}    
% \setcounter{figure}{4}
\begin{figure}[t]
\vspace{-0.1in}
  \centering
\begin{subfigure}{.435\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures/5(a)0930.png}  
    \caption{\small}% $\bz$ of datasets and graphs}
  %\caption{\small }
\end{subfigure}
\begin{subfigure}{.315\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures/5(b)0930.png}  
  %\vspace{-0.2in}
  \caption{\small}% $\bz$ of datasets}
 % \caption{\small }
\end{subfigure}
\hspace{-0.1in}
\begin{subfigure}{.225\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures/3_3.time_acc.PNG}
   \vspace{-0.28in}
    \caption{\small}
 % \caption{\small }
\end{subfigure}
%\hspace{-0.01in}
% \begin{subfigure}{.135\linewidth}
%   \centering
%     \subfloat{
%         \includegraphics[width=.5\linewidth]{figures/heatmap/3_2.heatmap_MNIST.png}
%     }
%     \subfloat{
%         \includegraphics[width=.5\linewidth]{figures/heatmap/3_2.heatmap_SVHN.png}
%     }
    
%     \subfloat{
%         \includegraphics[width=.5\linewidth]{figures/heatmap/3_2.heatmap_CIFAR10.png}
%     }
%     \subfloat{
%         \includegraphics[width=.5\linewidth]{figures/heatmap/3_2.heatmap_CIFAR100.png}
%     }
    
%     \subfloat{
%         \includegraphics[width=.5\linewidth]{figures/heatmap/3_2.heatmap_AIRCRAFT.png}
%     }
%     \subfloat{
%         \includegraphics[width=.5\linewidth]{figures/heatmap/3_2.heatmap_MetaD2A.png}
%     }
%     \addtocounter{subfigure}{-6}
%     \centering
%     \caption{\small $\bz$ heatmap}
%     %\caption{\small}
% \end{subfigure}
\vspace{-0.1in}
%\caption{\small \textbf{Qualitative Examples} The actual architectures and more examples are in \textbf{Suppl.~\ref{sec:quali_suppl}}}
\caption{\small \textbf{Qualitative Examples} \textbf{(a)} T-SNE vis. of $\bz$ of datasets (stars) and graphs (grey circles). \textbf{(b)} T-SNE vis. of $\bz$ of several datasets. \textbf{(c)} Mean Accuarcy over Search Time on unseen MetaImageNet tasks. The actual architectures and more examples of (a) and (b) are in the Section~\ref{sec:quali_suppl} of the Appendix.}%\textbf{(c)} Heatmap of $\bz$ from several datasets.}
\label{fig:quali}
\vspace{-0.2in}
\end{figure}


==> others/table_1_main.tex <==
\begin{table}[t!]
	\vspace{-0.25in}
	\caption{\small \textbf{Performance of our model and baselines on unseen MetaImageNet tasks.} We validate all models on 20 unseen tasks from MetaImageNet. We report the mean accuracies and $95\%$ confidence intervals.}\label{tbl:MetaImageNet} %The bold is the highest performance.}
	\vspace{-0.15in}
	\small
	\begin{center}
	     \resizebox{1.\linewidth}{!}{

		\begin{tabular}{lcccc|cc}
			\hline
			\multirow{2}{*}{Method} & \multirow{2}{*}{Transfer} & Search & Search & Params &\multicolumn{2}{c}{MetaImageNet}      \\
			 &  & Time (sec) & Expense (\textdollar) & (M) & Top-1 Accuracy & Top-5 Accuracy \\
			\hline
			\hline
			ResNet~\citep{He16}
			& N%/A
			& N/A
			& N/A
			& 0.86
			& 67.12\tiny$\pm$1.23
			& 91.03\tiny$\pm$0.68
			\\
			\hline
	         ENAS~\citep{pham2018efficient}
			& N%/A
			& 247479.12
			& 100.37
			& 0.07
			& 28.05\tiny$\pm$1.25
			& 63.90\tiny$\pm$1.54
			\\
			RSPS~\citep{li2020random}
			& N%/A
			& 11009.18
			& 4.46
 			& 0.28
			& 60.66\tiny$\pm$1.56
			& 89.37\tiny$\pm$0.90
			\\
			DARTS~\citep{liu2018darts}
			& N%/A
			& 9714.14
			& 3.94
 			& 0.10
			& 43.02\tiny$\pm$3.74
			& 76.70\tiny$\pm$2.72
			\\
			SETN~\citep{dong2019one}
			& N%/A
			& 30738.71
    		& 12.47
 			& 0.36
			& 60.87\tiny$\pm$1.54
			& 89.03\tiny$\pm$0.78
			\\
			GDAS~\citep{dong2019searching}
			& N%/A
			& 25272.03
			& 10.25
 			& 0.67
			& 64.59\tiny$\pm$1.36
			& 89.89\tiny$\pm$0.76
			\\
            PC-DARTS~\citep{xu2020pc}
			& N%/A
			& 10721.59
			& 8.39
	 	    & 0.44
			& 57.62\tiny$\pm$4.66
			& 83.60\tiny$\pm$4.97
			\\
			DrNAS~\citep{chen2020drnas}
			& N%/A
			& 10949.95
			& 4.44
 			& 1.00
			& 67.48\tiny$\pm$1.05
			& 91.36\tiny$\pm$0.63
			\\
			\hline
% 			Ours-RS
% 			& Y%/A
% 			& 0.1694 / 2291.36}
% 			& xx
% 			& 6$\bm{\times}$10$^{\bm{\shortminus5}}$}
% 			& 63.97\tiny$\pm$1.87
% 			& 89.37\tiny$\pm$0.87
% 			\\
			\textbf{MetaD2A (Ours)}
			& Y%MetaD2A
			& 27.03 / $26964.18^\text{\textdagger}$
			& 0.01/10.94
 			& 0.72
			& \textbf{69.36\tiny$\pm$2.16}
			& \textbf{91.91\tiny$\pm$1.21}
% 			& Y%MetaD2A
% 			& \textbf{0.0053 / 2291.36}
% 			& 0.7180
% 			& \textbf{2$\bm{\times}$10$^{\bm{\shortminus6}}$}%/\textbf{0.93}
% 			& \textbf{66.44\tiny$\pm$1.37}
% 			& \textbf{90.50\tiny$\pm$0.91}
% 			\\
% 			\textbf{Ours}
% 			& Y%MetaD2A
% 			& x.xxxx / xx.xx
% % 			& x.xxxx
% 			& xx
% 			& \textbf{70.72\tiny$\pm$1.38}
% 			& \textbf{92.68\tiny$\pm$0.78}
% 			& Y%MetaD2A
% 			& \textbf{0.0053 / 2291.36}
% 			& 0.7180
% 			& \textbf{2$\bm{\times}$10$^{\bm{\shortminus6}}$}%/\textbf{0.93}
% 			& \textbf{66.44\tiny$\pm$1.37}
% 			& \textbf{90.50\tiny$\pm$0.91}
			\\
			\hline
		\end{tabular} 		}
	\end{center}
	\small
	\vspace{-0.20in}
\end{table}

==> others/table_2_dataset.tex <==
\begin{savenotes}
\begin{table}[t!]
%\resizebox{0.9\linewidth}{!}{% 
	%\vspace{+0.2in}
	\caption{\small \textbf{Performance on multiple datasets} We transfer MetaD2A to target datasets after training on MetaImageNet, while other baselines are trained to search neural architectures for each dataset from scratch. We report accuracies\footnote{For some baseline models, we brought the results for CIFAR-10 and CIFAR-100 from NAS-Bench-201~\citep{dong2020bench} which performs the experiments with a single GeForce GTX 1080 Ti GPU.} with $95\%$ confidence intervals on multiple datasets and parameters on CIFAR10. %The bold is the highest performance.
	%For each model, we run $3$ independent trials and jointly test them over 10 episodes. We report mean accuracies and $95\%$ confidence intervals. Note that our model is trained on MetaD2A and is not trained again on CIFAR-10, CIFAR-100, and CUB-64-200, while all the baselines are retrained for each dataset.
	}
	\vspace{-0.15in}
	\small
	\begin{center}
     \resizebox{1.\linewidth}{!}{
	    \begin{tabular}{lc|cccccc}
	   	\hline
	    \multirow{2}{*}{Method} & Params & \multicolumn{6}{c}{Target Dataset} \\
                                & (M)
                                & MNIST & SVHN & CIFAR-10 & CIFAR-100 & Aircraft & Oxford-IIIT Pets &
	   % \begin{tabular}{lc|ccccc}
	   %	\hline
	   % \multirow{2}{*}{Method}  & Search & \multicolumn{5}{c}{Target Dataset} \\
    %                              & Time (sec)\footnote[2]{For baseline models, we brought search times for CIFAR-10 and CIFAR-100 from NAS-Bench-201~\citep{dong2020bench} which performs all experiments with a single GeForce GTX 1080 Ti GPU.} 
    %                             & MNIST & SVHN & CIFAR-10 & CIFAR-100 & Aircraft
	    \hline
	    \hline
	    Optimal
	    & -
	    & -
	    & -
	    & 94.37
	    & 73.51
	    & -
	    & -
	   \\
	    ResNet~\citep{He16}
	    & 0.86
	    & 99.67\tiny$\pm$0.01
	    & 96.13\tiny$\pm$0.19
	    & 93.97\tiny$\pm$0.00
	    & 70.86\tiny$\pm$0.00
	    & 47.01\tiny$\pm$1.16
	    & 25.58\tiny$\pm$3.43
	    \\
	    \hline
	    REA~\citep{real2019regularized}
	    & -
	    & -
	    & -
	    & 93.92\tiny$\pm$0.30
	    & 71.84\tiny$\pm$0.99
	    & -
	    & -
	    \\
	    RS~\citep{bergstra2012random}
	    & -
	    & -
	    & -
	    & 93.70\tiny$\pm$0.36
	    & 71.04\tiny$\pm$1.07
	    & -
	    & -
	    \\
	   REINFORCE~\citep{williams1992simple}
	    & -
	    & -
	    & -
	    & 93.85\tiny$\pm$0.37
	    & 71.71\tiny$\pm$1.09
	    & -
	    & -
	    \\
	    BOHB~\citep{falkner2018bohb}
	    & -
	    & -
	    & -
	    & 93.61\tiny$\pm$0.52
	    & 70.85\tiny$\pm$1.28
	    & -
	    & -
	    \\
	    \hline
	   DVAE~\citep{zhang2019d}
	   & 0.86
	   & -
	   & -
	   & 85.53\tiny$\pm$1.31 % seed 10번
	   & 51.10\tiny$\pm$3.99 % seed 10번
	   & -
	   & -
	   \\
	    RSPS~\citep{li2020random}
	    & -
	    & 99.63\tiny$\pm$0.02
	    & 96.17\tiny$\pm$0.12
	    & 84.07\tiny$\pm$3.61
	    & 52.31\tiny$\pm$5.77
	    & 42.19\tiny$\pm$3.88
	    & 22.91\tiny$\pm$1.65
	    %& 14.33\tiny$\pm$1.66
	    %& xx.xx\tiny$\pm$x.xx
	    \\
	    DARTS~\citep{liu2018darts}
	    & -
	    & 98.82\tiny$\pm$0.69
	    & 65.71\tiny$\pm$25.88
	    & 54.30\tiny$\pm$0.00
	    & 15.61\tiny$\pm$0.00
	    & 22.50\tiny$\pm$0.04 % 22.53\tiny$\pm$0.03
	    & 18.14\tiny$\pm$5.00
	    %& 18.26\tiny$\pm$0.78
	    %& 6.09\tiny$\pm$3.49
	    \\
	    SETN~\citep{dong2019one}
	    & -
	    & 99.69\tiny$\pm$0.04
	    & 96.02\tiny$\pm$0.12
	    & 87.64\tiny$\pm$0.00
	    & 59.05\tiny$\pm$0.24
	    & 44.84\tiny$\pm$3.96 % 44.62\tiny$\pm$5.44
	    & 25.17\tiny$\pm$1.68
	    %& 10.42\tiny$\pm$3.97
	    %& 10.71\tiny$\pm$0.98
	    \\
	    GDAS~\citep{dong2019searching}
	    & -
	    & 99.64\tiny$\pm$0.04
	    & 95.57\tiny$\pm$0.57
	    & 93.61\tiny$\pm$0.09
	    & 70.70\tiny$\pm$0.30
	    & 53.52\tiny$\pm$0.48
	    & 24.02\tiny$\pm$2.75
	    %& 8.19\tiny$\pm$2.91
	    %& 10.98\tiny$\pm$1.75
	    \\
	   PC-DARTS~\citep{xu2020pc}
	   & 1.18
	   & 99.66\tiny$\pm$0.04
	   & 95.40\tiny$\pm$0.67
	   & 93.19\tiny$\pm$0.69
	   & 68.89\tiny$\pm$0.23
	   & 26.33\tiny$\pm$3.40
	   & 19.25\tiny$\pm$8.52
	   \\
	   DrNAS~\citep{chen2020drnas}
	   & 1.53
	   & 99.60\tiny$\pm$0.04
	   & 96.28\tiny$\pm$0.01
	   & 93.76\tiny$\pm$0.00
	   & 71.50\tiny$\pm$0.75
	   & 40.45\tiny$\pm$9.06
	   & 26.73\tiny$\pm$2.61
	   \\
	   FNA~\citep{fang2020fast}
	   & 0.07
	   & 99.51\tiny$\pm$0.16
	   & 94.19\tiny$\pm$0.12
	   & 70.41\tiny$\pm$0.77
	   & -
	   & 26.43\tiny$\pm$3.37
	   & 13.57\tiny$\pm$0.41
	   \\
	   \hline
	   %% Ours-RS
	   %% & MetaD2A
	   %% & 0.1694}
	   %% & xx.xx
	   %% & 99.46\tiny$\pm$0.24
	   %% & 57.48\tiny$\pm$42.62
	   %% & 86.14\tiny$\pm$6.90
	   %% & 62.11\tiny$\pm$3.72
	   %% & 50.89\tiny$\pm$1.63
	   %% \\
	   %% \textbf{Ours (no pp.)}
	   %% & MetaD2A
	   %% & xx
	   %% & xx.xx
	   %% & xx
	   %% & xx
	   %% & xx
	   %% & xx
	   %% & xx \\
	    \textbf{MetaD2A (Ours)}
	    & 1.05
	    & \textbf{99.70\tiny$\pm$0.18}
	    & \textbf{96.56\tiny$\pm$0.13}
	    & \textbf{94.37\tiny$\pm$0.01}
	    & \textbf{73.51\tiny$\pm$0.00}
	    & \textbf{60.31\tiny$\pm$0.74}
	    & \textbf{38.74\tiny$\pm$0.08}
	    \\
	   % \textbf{Ours (N=1)}
	   %% & MetaD2A
	   %% & xxxx
	   %%% & x.xxxx
	   %% & 99.68\tiny$\pm$0.00
	   %% & \textbf{99.57\tiny$\pm$0.59}
	   %% & 93.12\tiny$\pm$0.58
	   %% & 70.34\tiny$\pm$0.61
	   %% & \textbf{60.41\tiny$\pm$3.05} \\	   
	   %% \textbf{Ours}
	   %% & MetaD2A
	   %% & xxxx
	   %%% & x.xxxx
	   %% & \textbf{99.73\tiny$\pm$0.64}
	   %% & \textbf{99.57\tiny$\pm$0.59}
	   %% & \textbf{94.37\tiny$\pm$0.01}
	   %% & \textbf{73.51\tiny$\pm$0.00}
	   %% & \textbf{60.41\tiny$\pm$3.05}
	   %% & \textbf{0.03}
	   %% & 0.8917
	   %% & 99.62\tiny$\pm$0.16
	   %% & \textbf{96.18\tiny$\pm$0.16}
	   %% & \textbf{94.37\tiny$\pm$0.01}
	   %% & \textbf{73.51\tiny$\pm$0.00}
	   %% & 53.15\tiny$\pm$0.82}
	   % \\
	    \hline
	    \end{tabular}
	    }
	\end{center}
	\small
	\label{tbl:2}
	\vspace{-0.1in}
	
\end{table}
\end{savenotes}


% \begin{savenotes}
% \begin{table}[t!]
% %\resizebox{0.9\linewidth}{!}{% 
% 	%\vspace{+0.2in}
% 	\caption{\small \textbf{Performance on multiple datasets} We transfer ours to target datasets after training on MetaImageNet, while other baselines are trained for each dataset from scratch. Note that it does mean ours only requires inference time but the others require the whole search time. We report the mean accuracies and $95\%$ confidence intervals over $3$ runs. The bold is the highest performance.
% 	%For each model, we run $3$ independent trials and jointly test them over 10 episodes. We report mean accuracies and $95\%$ confidence intervals. Note that our model is trained on MetaD2A and is not trained again on CIFAR-10, CIFAR-100, and CUB-64-200, while all the baselines are retrained for each dataset.
% 	}
% 	\vspace{-0.1in}
% 	\small
% 	\begin{center}
%      \resizebox{1.\linewidth}{!}{

% 	    \begin{tabular}{lcc|ccccc}
% 	   	\hline
% 	    \multirow{2}{*}{Method} & Source  & Search & \multicolumn{5}{c}{Target Dataset} \\
%                                 & Dataset & Time (sec)\footnote[2]{For baseline models, we brought search times for CIFAR-10 and CIFAR-100 from NAS-Bench-201~\citep{dong2020bench} which performs all experiments with a single GeForce GTX 1080 Ti GPU.} 
%                                 & MNIST & SVHN & CIFAR-10 & CIFAR-100 & Aircraft & 
% 	    \hline
% 	    \hline
% 	    Optimal
% 	    & -
% 	   % & - 
% 	    & -
% 	    & -
% 	    & -
% 	    & 94.37
% 	    & 73.51
% 	    & -
% 	    \\
% 	    ResNet%~\citep{He16}
% 	    & N/A
% 	    & N/A
% 	   % & 0.8600
% 	    & 99.62\tiny$\pm$0.16
% 	    & xx.xx\tiny$\pm$x.xx
% 	    & 93.97\tiny$\pm$0.00
% 	    & 70.86\tiny$\pm$0.00
% 	    & 47.77\tiny$\pm$2.71
% 	    \\
% 	    \hline
% 	    REA
% 	    & N/A
% 	    & 0.02
% 	   % & -
% 	    & -
% 	    & -
% 	    & 93.92\tiny$\pm$0.30
% 	    & 71.84\tiny$\pm$0.99
% 	    & -
% 	    \\
% 	   RS
% 	   & N/A
% 	    & 0.01
% 	   % & -
% 	    & -
% 	    & -
% 	    & 93.70\tiny$\pm$0.36
% 	    & 71.04\tiny$\pm$1.07
% 	    & -
% 	    \\
% 	   REINFORCE
% 	   & N/A
% 	    & 0.12
% 	   % & -
% 	    & -
% 	    & -
% 	    & 93.85\tiny$\pm$0.37
% 	    & 71.71\tiny$\pm$1.09
% 	    & -
% 	    \\
% 	   BOHB
% 	   & N/A
% 	    & 3.59
% 	   % & -
% 	    & -
% 	    & -
% 	    & 93.61\tiny$\pm$0.52
% 	    & 70.85\tiny$\pm$1.28
% 	    & -
% 	    \\
% 	    \hline
% 	   DVAE
% 	   & N/A
% 	   & 79358.61
% 	   %& xx.xx
% 	   & -
% 	   & -
% 	   & 85.53\tiny$\pm$1.31 % seed 10번
% 	   & 51.10\tiny$\pm$3.99 % seed 10번
% 	   & -
% 	   \\
% 	    RSPS%~\citep{li2020random}
% 	    & N/A
% 	    & 8007.13
% 	   % & 0.3183
% 	    & 99.68\tiny$\pm$0.06
% 	    & 96.15\tiny$\pm$0.17
% 	    & 84.07\tiny$\pm$3.61
% 	    & 52.31\tiny$\pm$5.77
% 	    & 42.32\tiny$\pm$5.16
% 	    %& 14.33\tiny$\pm$1.66
% 	    %& xx.xx\tiny$\pm$x.xx
% 	    \\
% 	    DARTS%~\citep{liu2018darts}
% 	    & N/A
% 	    & 11625.77
% 	   % & 0.0877
% 	    & 98.77\tiny$\pm$0.90
% 	    & 65.62\tiny$\pm$33.60
% 	    & 54.30\tiny$\pm$0.00
% 	    & 15.61\tiny$\pm$0.00
% 	    & 22.53\tiny$\pm$0.03
% 	    %& 18.26\tiny$\pm$0.78
% 	    %& 6.09\tiny$\pm$3.49
% 	    \\
% 	   DrNAS
% 	   & N/A
% 	   & 23003.50
% 	   %& 1.3341
% 	   & 99.57\tiny$\pm$0.01
% 	   & 96.34\tiny$\pm$0.01
% 	   & 93.76\tiny$\pm$0.00
% 	   & 71.5\tiny$\pm$0.75
% 	   & 40.84\tiny$\pm$0.94
% 	   \\
% 	   PC-DARTS
% 	   & N/A
% 	   & 25653.00
% 	   %& xx.xx
% 	   & xx.xx
% 	   & xx.xx
% 	   & 93.67\tiny$\pm$0.15
% 	   & 66.72\tiny$\pm$4.86
% 	   & xx.xx
% 	   \\
% 	    SETN%~\citep{dong2019one}
% 	    & N/A
% 	    & 34139.53
% 	   % & 0.4928
% 	    & \textbf{99.70\tiny$\pm$0.03}
% 	    & 95.71\tiny$\pm$0.80
% 	    & 87.64\tiny$\pm$0.00
% 	    & 59.05\tiny$\pm$0.24
% 	    & 44.62\tiny$\pm$5.44
% 	    %& 10.42\tiny$\pm$3.97
% 	    %& 10.71\tiny$\pm$0.98
% 	    \\
% 	   % NASwT
% 	   % & N/A
% 	   % & 17.40
% 	   % & -
% 	   % & -
% 	   % & 91.78\tiny$\pm$1.45
% 	   % & 67.05\tiny$\pm$2.89
% 	   % & -
% 	   % %& 11.16\tiny$\pm$3.58
% 	   % %& 11.10\tiny$\pm$1.32
% 	   % \\
% 	    GDAS%~\citep{dong2019searching}
% 	    & N/A
% 	    & 31609.80
% 	   % & 0.5566
% 	    & 99.64\tiny$\pm$0.05
% 	    & 95.68\tiny$\pm$0.58
% 	    & 93.61\tiny$\pm$0.09
% 	    & 70.70\tiny$\pm$0.30
% 	    & 53.74\tiny$\pm$0.64
% 	    %& 8.19\tiny$\pm$2.91
% 	    %& 10.98\tiny$\pm$1.75
% 	    \\
% 	   % CDARTS
% 	   % & N/A
% 	   % & xx.xx
% 	   % & xx.xx
% 	   % & xx.xx-
% 	   % & \textbf{94.02\tiny$\pm$0.31}
% 	   % & \textbf{71.92\tiny$\pm$1.30}
% 	   % & xx.xx
% 	   % \\

% 	   %\hline
% 	   \hline
% 	   % Ours-RS
% 	   % & MetaD2A
% 	   % & 0.1694}
% 	   % & xx.xx
% 	   % & 99.46\tiny$\pm$0.24
% 	   % & 57.48\tiny$\pm$42.62
% 	   % & 86.14\tiny$\pm$6.90
% 	   % & 62.11\tiny$\pm$3.72
% 	   % & 50.89\tiny$\pm$1.63
% 	   % \\
% 	   % Ours-LSTM
% 	   % & MetaD2A
% 	   % & xx.xx
% 	   % & xx.xx\tiny$\pm$x.xx
% 	   % & xx.xx\tiny$\pm$x.xx
% 	   % & xx.xx\tiny$\pm$x.xx
% 	   % & xx.xx\tiny$\pm$x.xx
% 	   % & xx.xx\tiny$\pm$x.xx
% 	   % %& 11.16\tiny$\pm$3.58
% 	   % %& 11.10\tiny$\pm$1.32
% 	   % \\
% 	   % \textbf{Ours (no pp.)}
% 	   % & MetaD2A
% 	   % & xx
% 	   % & xx.xx
% 	   % & xx
% 	   % & xx
% 	   % & xx
% 	   % & xx
% 	   % & xx \\
% 	    \textbf{Ours}
% 	    & MetaImageNet
% 	    & 22.47
% 	   % & x.xxxx
% 	    & \textbf{99.70\tiny$\pm$0.18}
% 	    & \textbf{96.56\tiny$\pm$0.13}
% 	    & \textbf{94.37\tiny$\pm$0.01}
% 	    & \textbf{73.51\tiny$\pm$0.00}
% 	    & \textbf{60.31\tiny$\pm$0.74} 	   
% 	   % \textbf{Ours (N=1)}
% 	   % & MetaD2A
% 	   % & xxxx
% 	   %% & x.xxxx
% 	   % & 99.68\tiny$\pm$0.00
% 	   % & \textbf{99.57\tiny$\pm$0.59}
% 	   % & 93.12\tiny$\pm$0.58
% 	   % & 70.34\tiny$\pm$0.61
% 	   % & \textbf{60.41\tiny$\pm$3.05} \\	   
% 	   % \textbf{Ours}
% 	   % & MetaD2A
% 	   % & xxxx
% 	   %% & x.xxxx
% 	   % & \textbf{99.73\tiny$\pm$0.64}
% 	   % & \textbf{99.57\tiny$\pm$0.59}
% 	   % & \textbf{94.37\tiny$\pm$0.01}
% 	   % & \textbf{73.51\tiny$\pm$0.00}
% 	   % & \textbf{60.41\tiny$\pm$3.05}
% 	   % & \textbf{0.03}
% 	   % & 0.8917
% 	   % & 99.62\tiny$\pm$0.16
% 	   % & \textbf{96.18\tiny$\pm$0.16}
% 	   % & \textbf{94.37\tiny$\pm$0.01}
% 	   % & \textbf{73.51\tiny$\pm$0.00}
% 	   % & 53.15\tiny$\pm$0.82}
% 	    \\
% 	    \hline
% 	    \end{tabular}
% 	    }
% 	\end{center}
% 	\small
% 	\label{tbl:2}
% 	\vspace{-0.2in}
	
% \end{table}
% \end{savenotes}

==> others/table_2_time.tex <==
\begin{savenotes}
\begin{table}[t!]
	\caption{\small \textbf{Architecture Search Time on multiple datasets} We report architecture search time(s) of each model on various datasets. After once meta-trained on MetaImageNet, we transfer MetaD2A to target datasets, while other baselines are trained to search neural architectures for each dataset from scratch. %\footnote[3]{For some baseline models, we brought search times from NAS-Bench-201~\citep{dong2020bench} which performs all experiments with a single GeForce GTX 1080 Ti GPU.}
	}
	\vspace{-0.15in}
	\small
	\begin{center}
     \resizebox{1.\linewidth}{!}{
	    \begin{tabular}{l|cccccc}
	   	\hline
	    \multirow{2}{*}{Method} %& Pre-/Meta-train 
	    & \multicolumn{6}{c}{Target Dataset} \\
	                            %& (s)
                                & MNIST & SVHN & CIFAR-10 & CIFAR-100 & Aircraft & Oxford-IIIT Pets &
	    \hline
	    \hline
	    RSPS~\citep{li2020random}
	    %& N/A
	    & 22457.20
	    & 27962.50
	    & 10200.10
	    & 18841.70
	    & 18697.40
	    & 3360.20
	    \\
	    DARTS~\citep{liu2018darts}
	    %& N/A
	    & 22398.40
	    & 26900.60
	    & 8007.13
	    & 18203.70
	    & 3624.70
	    & 2469.40
	    \\
	    SETN~\citep{dong2019one}
	    %& N/A
	    & 69656.20 
	    & 85189.60 
	    & 30220.70 
	    & 58808.70 
	    & 18564.40 
	    & 8625.20 
	    \\
	    GDAS~\citep{dong2019searching}
	    %& N/A
	    & 60186.50 
	    & 71595.00 
	    & 25077.20 
	    & 51580.00 
	    & 18508.20 
	    & 6965.40 
	    \\
	   PC-DARTS~\citep{xu2020pc}
	   %& N/A
	    & 24857.80 
	    & 31124.50 
	    & 10395.00 
	    & 19951.50 
	    & 3524.30 
	    & 2844.60 
	   \\
	   DrNAS~\citep{chen2020drnas}
	   %& N/A
	    & 44131.00 
	    & 52791.00 
	    & 21760.00 
	    & 34529.00 
	    & 32422.00 
	    & 6019.50 
	   \\
	   FNA~\citep{fang2020fast}
	   %& 6856
	   	& 22830.40%19634.14
	    & 27087.90%15169.22
	    & 9462.80%9462.80 
	    & -
	    & 3972.80%3178.24
	    & 2619.50%2357.55
	   \\
	   \hline
	    \textbf{MetaD2A (Ours)}
	    %& 26964.18
	    & \textbf{32.95} 
	    & \textbf{30.20} 
	    & \textbf{22.47} %26.98
	    & \textbf{68.58} 
	    & \textbf{34.51} 
	    & \textbf{38.79} 
	    \\
	    \hline
	    \end{tabular}
	    }
	\end{center}
	\small
	\label{tbl:2_time}
	\vspace{-0.1in}
	
\end{table}
\end{savenotes}


==> others/table_3_fewshot.tex <==
\begin{table}[h]
	\caption{\small \textbf{Performance of our model and baselines on Few-shot classification tasks.} }\label{tbl:fewshot} %The bold is the highest performance.}
	\vspace{-0.1in}
	\small
	\begin{center}
	     \resizebox{1.\linewidth}{!}{

		\begin{tabular}{lccc|cc}
			\hline
			\multirow{2}{*}{Method} & \multirow{2}{*}{NAS} & Search & \multirow{2}{*}{Params} &\multicolumn{2}{c}{MiniImageNet}      \\
			 & & Time (Hours) &  & 5-way 1-shot & 5-way 5-shot \\
			\hline
			\hline
			MAML~\citep{finn2017model}
			& 
			& N/A
			& 30K
			& 48.7\tiny$\pm$1.8
			& 63.1\tiny$\pm$0.9
			\\
	        REPTILE~\citep{nichol2018first}
			& 
			& N/A
			& 30K
			& 50.0\tiny$\pm$0.3
			& 66.0\tiny$\pm$0.6
			\\
	        AutoMeta
			& \checkmark
			& -/2400
			& 100K
			& 57.6\tiny$\pm$0.2
			& 74.7\tiny$\pm$0.2
			\\
	        T-NAS++~\citep{lian2019towards}
			& \checkmark
			& 1.5 or 7.8/3600
			& 27K
			& 54.1\tiny$\pm$1.4
			& 69.6\tiny$\pm$0.9
			\\
	        BASE~\citep{shaw2019meta}
			& \checkmark
			& -/-
			& 1.2M
			& -
			& 66.2\tiny$\pm$0.7
			\\
	        TADAM
			& 
			& N/A
			& 12M
			& 58.5\tiny$\pm$0.3
			& 76.7\tiny$\pm$0.3
			\\
	        LEO~\citep{rusu2018leo}
			& 
			& N/A
			& 36.5M
			& 61.8\tiny$\pm$0.1
			& 77.6\tiny$\pm$0.1
			\\
	        MetaOptNet
			& 
			& N/A
			& 12M
			& 61.1\tiny$\pm$0.6
			& 77.4\tiny$\pm$0.5
			\\
	        MetaNAS~\citep{elsken2020meta}
			& \checkmark
			& -/168
			& 1M
			& 61.7\tiny$\pm$0.3
			& 78.8\tiny$\pm$0.2
			\\
			\hline
	        MetaD2A (Ours)
			& \checkmark
			& xx
			& xx
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			\\
			\hline
		\end{tabular} 		}
	\end{center}
	\small
	\vspace{-0.20in}
\end{table}

==> others/table_abl.tex <==
% \begin{minipage}[t!]{\textwidth}
% 	%\vspace{0.08in}
% 	\begin{minipage}{0.42\textwidth}
% 	    \vspace{0.05in}
% 		\centering 
% 		\small
% 		\resizebox{1\textwidth}{!}{
% 	    \begin{tabular}{l|cc}
% 	   % \toprule 
% 	   \hline
% 	   \multicolumn{1}{c|}{Source Dataset} & \multicolumn{2}{c}{Target Dataset} &
% 	   \multicolumn{1}{c|}{MetaImageNet} & \multicolumn{1}{c}{CIFAR10} &
% 	   \multicolumn{1}{c}{CIFAR100} &
% 	   %Model & Top 1 & Top 10 & Top 100 
% 	   %         & Top 1 & Top 10 & Top 100\\
% 	   \hline
% 	  Optimal                       & 
%       94.37                         & 
%       73.51                       \\   
%       \hline
%       Random                       & 
%       93.52\tiny$\pm$0.25          & 
%       70.71\tiny$\pm$0.53         \\   
%       %RLV                       & 
%       %92.82\tiny$\pm$0.82          &
%       %93.85\tiny$\pm$0.38          & 
%       %94.23\tiny$\pm$0.19          & 
%       %68.88\tiny$\pm$1.63          &
%       %71.53\tiny$\pm$1.06          & 
%       %73.20\tiny$\pm$0.33         \\   
%       Random w/ PP.                & 
%       94.02\tiny$\pm$0.11          & 
%       72.83\tiny$\pm$0.48          \\   
%       MetaD2A w/o PP.               & 
%       94.09\tiny$\pm$0.22          & 
%       72.76\tiny$\pm$0.55          \\
%       %RLV+PP                    & 
%       %92.38\tiny$\pm$2.21          &
%       %94.13\tiny$\pm$0.20          & 
%       %\textbf{94.37\tiny$\pm$0.01} & 
%       %68.55\tiny$\pm$3.69          &
%       %72.79\tiny$\pm$0.55          & 
%       %73.46\tiny$\pm$0.12          \\ 
%       MetaD2A                       & 
%       \textbf{94.37\tiny$\pm$0.01} & 
%       \textbf{73.51\tiny$\pm$0.00} \\  
% 	  \hline
% 	   % \bottomrule
% 	    \end{tabular}
% 		}
% % 	\vspace{-0.12in}
% 	\captionof{table}{\small Ablation study of MetaD2A }\label{tbl:abl}
% 	\end{minipage}
% 	\begin{minipage}{0.59\textwidth}
% 		%\vspace{-0.1in}
% 		\centering
% 		\includegraphics[height=2.7cm]{figures/4_pp_abl_cifar10.png}
%         \includegraphics[height=2.7cm]{figures/4_pp_abl_cifar100.png}
% 		\vspace{-0.1in}
% 		\captionof{figure}{\small Accuracy over the number of architecture sampling }
% 		\label{fig:abl}
% 	\end{minipage}
% 	\vspace{-0.05in}
% \end{minipage}

\begin{minipage}[t!]{\textwidth}
	%\vspace{0.08in}
	\begin{minipage}{0.49\textwidth}
	    \vspace{0.05in}
		\centering 
		\small
		\resizebox{1\textwidth}{!}{
	    \begin{tabular}{l|ccc}
	   % \toprule 
	   \hline
	   \multicolumn{1}{c|}{Source Dataset} & \multicolumn{3}{c}{Target Dataset} &
	   \multicolumn{1}{c|}{MetaImageNet} & \multicolumn{1}{c}{CIFAR10} &
	   \multicolumn{1}{c}{CIFAR100} & \multicolumn{1}{c}{Aircraft} &
	   %Model & Top 1 & Top 10 & Top 100 
	   %         & Top 1 & Top 10 & Top 100\\
	   \hline
	  Optimal                       & 
      94.37                         & 
      73.51                         &
      -                            \\
      \hline
      Random                       & 
      93.52\tiny$\pm$0.25          & 
      70.71\tiny$\pm$0.53          &
      38.15\tiny$\pm$0.99
         \\   
      Random w/ PP.                & 
      94.02\tiny$\pm$0.11          & 
      72.83\tiny$\pm$0.48          &
      53.39\tiny$\pm$3.13
         \\   
      MetaD2A w/o PP.               & 
      94.09\tiny$\pm$0.22           & 
      72.76\tiny$\pm$0.55           &
      53.45\tiny$\pm$3.27          \\   

      MetaD2A                       & 
      \textbf{94.37\tiny$\pm$0.01} & 
      \textbf{73.51\tiny$\pm$0.00} &
      \textbf{60.31\tiny$\pm$0.73}        \\   
	  \hline
	    \end{tabular}
		}
% 	\vspace{-0.12in}
	\captionof{table}{\small Ablation study of MetaD2A }\label{tbl:abl_old}
	\end{minipage}
	\begin{minipage}{0.50\textwidth}
		%\vspace{-0.1in}
		\centering
		\includegraphics[height=2.4cm]{figures/4_pp_abl_cifar10.png}
        \includegraphics[height=2.4cm]{figures/4_pp_abl_cifar100.png}
		\vspace{-0.1in}
		\captionof{figure}{\small Accuracy over the number of arch. sampling }
		\label{fig:abl}
	\end{minipage}
	%\vspace{-0.05in}
\end{minipage}


==> others/table_pp_abl.tex <==
\begin{wraptable}{r}{0.45\textwidth}
\vspace{-0.15in}
\resizebox{0.45\textwidth}{!}{
\vspace{-0.25in}

\begin{minipage}[h!]{\textwidth}
% 	\begin{minipage}{0.3\textwidth}
% 	    \vspace{0.05in}
% 		\centering 
% 		\small
% 		\resizebox{1\textwidth}{!}{
%     \begin{tabular}{c|c}
% 	   % \toprule 
% 	   \hline
% 	   	\multicolumn{1}{c}{Training} &  \multicolumn{1}{c}{Pearson} \\
%       \multicolumn{1}{c}{Task size} &  \multicolumn{1}{c}{Corr. Coeff.} \\
% 	   \hline
% 	   \hline
%         1000       &
% 	    0.6496    \\
%         1500       &
% 	    0.7312    \\
%       2000        &
% 	   0.7476      \\
%       2500        &
% 	   0.7565      \\
%       3000        &
% 	   0.7669      \\
%       3752         &
% 	   \textbf{0.7976}\\
% 	    \hline
% 	   % \bottomrule
% 	    \end{tabular}
% 		}
% % 	\vspace{-0.12in}
% 	\captionof{table}{\small} %Abl. study }
% 	\end{minipage}
	\begin{minipage}{1.0\textwidth}
		%\vspace{-0.1in}
		\centering
		\includegraphics[height=0.485\textwidth]{figures/5_pp_abl_datasize_CIAFR10.png}
        \includegraphics[height=0.485\textwidth]{figures/5_pp_abl_datasize_CIAFR100.png}
		\vspace{-0.1in}
		\captionof{figure}{\small }
		\label{fig:ood}
	\end{minipage}
	\vspace{-0.05in}
\end{minipage}
}
\end{wraptable}

==> others/table_pp_abl2.tex <==
\begin{wraptable}{r}{0.38\textwidth}
\vspace{-0.05in}
\resizebox{0.38\textwidth}{!}{
\vspace{-0.25in}

\begin{tabular}{cccccc|c}
	   % \toprule 
	   \hline
	   	\multicolumn{2}{c}{Input Type} & \multicolumn{3}{c}{Encoder} & \multicolumn{1}{c|}{Decoder} & \multicolumn{1}{c}{Pearson} \\
       %\cmidrule(c){1-2} \cmidrule(c){3-4} \cmidrule(c){5-5}
	   %\hline
       \multicolumn{1}{c}{Data} & \multicolumn{1}{c}{Graph} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{Set} & \multicolumn{1}{c}{Hier.} & \multicolumn{1}{c|}{Bi-dir.} & \multicolumn{1}{c}{Corr. Coeff.} \\
	   \hline
	   \hline
        %\midrule
	    \checkmark &
	               &
        \checkmark &
	               &
	               &
	               &
	    0.3699
	   \\
                  &
	    \checkmark &
	    \checkmark &
	               &
	               &
	               &
	   0.6518
	   \\
        \checkmark &
	    \checkmark &
        \checkmark &
	               &
	               &
	               &
	   0.7299
	   \\
        \checkmark &
	    \checkmark &
	               &
	    \checkmark &
	               &
	               &
	   0.7647
	   \\
      \checkmark &
	   \checkmark &
	              &
	   \checkmark &
	   \checkmark &
	              &

	   0.7663
	   \\
      \checkmark &
	   \checkmark &
	              &
	   \checkmark &
	   \checkmark &
	   \checkmark &
	   \textbf{0.7976}
	   \\
	    \hline
	   % \bottomrule
	    \end{tabular}
	    }
\vspace{-0.1in}
\caption{\small {Ablation Study of Predictor.} }\label{tbl:pp_abl2}
\vspace{-0.2in}
\end{wraptable}

==> others/table_vae.tex <==
\begin{wraptable}{r}{0.34\textwidth}
\vspace{-0.1in}
\resizebox{0.34\textwidth}{!}{
\vspace{-0.25in}

\begin{tabular}{ccc}
	   % \toprule 
	   \hline
       \multicolumn{1}{c}{Validity} & \multicolumn{1}{c}{Uniqueness} & \multicolumn{1}{c}{Novelty}\\
	   \hline
	    1.0000 &
	    0.3519 &
	    0.6731 \\
	    \hline
	    \end{tabular}
	    }
\vspace{-0.1in}
\caption{\small {Generative Abilities}}\label{tbl:vae}
\vspace{-0.2in}
\end{wraptable}

==> sections/4_method.tex <==
\section{Method}
\label{sec:method}
\vspace{-0.1in}

Our goal is to output a high-performing neural architecture for a given dataset rapidly by learning the prior knowledge obtained from the rich database consisting of datasets and its neural architectures. To this end, we propose Meta Dataset-to-Architecture (MetaD2A) framework which learns the cross-modal latent space of datasets and their neural architectures. Further, we introduce a meta-performance predictor, which predicts accuracies of given architectures on an unseen input dataset to select the best neural architecture for the dataset. Figure~\ref{fig:overview} illustrates the overview of our framework.

\input{Figure_tex/figure_overview}


% $\mX^\tau = \{\mX^\tau_c\}_{c=1}^C$
To formally define the problem, let us assume that we have a database of $N_\tau$ number of tasks, where we randomly obtain tasks $\tau$ from task distribution $p(\tau)$ to train for the model.  Each task $\tau = \{ \D, \G, s \}$ consists of a dataset $\D = \{ \mX, \mY \}$, where $\mX = \{\mX_c\}_{c=1}^C$ and $\mY = \{\mY_c\}_{c=1}^C$ are the set of instances and target labels of $C$ classes respectively, a neural architecture represented as a Directed Acyclic Graph (DAG) $\G=\{ \V, \mathcal{E} \}$, and an accuracy $\bm{s}$ obtained from the neural architecture $\G$ trained on $\D$. Each node $v \in \V$ of $\G$ then represents a computational operator (e.g. 3-by-3 convolution, mean-pooling, \dots) and each edge $(u, v) \in \mathcal{E}$ represents a computation flow from an output of the operator $u$ to input of the operator $v$. The whole framework consists of a set encoder, a graph decoder, and a meta-performance predictor parameterized by $\bm{\phi}$, $\bm{\theta}$, and $\bm{\omega}$, respectively. The dataset $\D$ is embedded into a latent space $\mathcal{Z}$ as a vector $\bz$ through the set encoder $q_{\bm{\phi}}$ and then the graph decoder $p_{\bm{\theta}}$ estimates the distribution and generates a new graph $\tilde \G$ from $\bz$ which are sampled from prior the $p(\bz)$. We learn both components $q_{\bm{\phi}} (\bz|\D)$ and $p_{\bm{\theta}} (\G|\bz)$, generalizing over the task distribution $p(\tau)$. After training, for an unseen dataset ${\hat{\D}}$, our model with $\bm{\theta}$ and $\bm{\phi}$ can easily generate DAGs $\{ {\hat{\G_i}}\}_{i=1}^{n_s}$ as candidates, where $n_s$ is the number of sampled architectures. This is done by decoding the latent embeddings $\{\hat{\bz}_i | \hat{\bz}_i \in \mathcal{Z} \}_{i=1}^{n_s}$ sampled from the prior $p(\bz)$ consisting of $\hat{\bm{\mu}}$ and $\hat{\bm{\sigma}}$ generated from the set encoder for given $\hat{\D^}$. The predictor $f_{\bm{\omega}}(s|\mathcal{D}, \mathcal{G})$ is also learned from the task distribution $p(\tau)$ in the meta-training stage and then selects the best performing neural architecture for ${\hat{\D^}}$ from $\{ \hat{\G_i} \}_{i=1}^{n_s}$ based on their predicted accuracies $\{ \hat{s_i} \}_{i=1}^{n_s}$ in the meta-test.


%We first introduce the set encoder and the graph decoder in Section~\ref{sec:encoder} and Section~\ref{sec:decoder}, respectively. Optimization strategy for accumulating knowledge of rich model database is introduced in Section~\ref{sec:optimization}. The performance predictor is introduced in Section~\ref{sec:predictor}.

%\input{others/figure_model_component.tex}


\vspace{-0.05in}
\subsection{Learning to Generate Graphs from Datasets}
\label{sec:generator}
\vspace{-0.05in}

\paragraph{Dataset Encoding} To compress the entire instances from a dataset $\D$ into a single latent code $\bz$, the set encoder should process input sets of any size and summarize consistent information agnostically to the order of the instances (permutation-invariance). While simple functions such as mean/sum-pooling can fulfill those requirements, they cannot model high-order interactions between the set elements to accurately generate complex DAGs such as neural architectures. Further, those non-hierarchical poolings consider all elements equally, and thus cannot accurately model individual classes in the given dataset, which may lead to poor performance~\citep{lee2020l2b}.

%\input{others/figure_hier_setpooling}
Therefore, we introduce a novel \textbf{Hierarchical Set Pooling} for dataset encoding which stacks two permutation-invariant encoders with learnable parameters, that can extract information related to generating set-conditioned DAGs. The lower-level intra-class encoder captures the class prototypes that reflect label information, and the high-level inter-class encoder considers the relationship between class prototypes and aggregates them into a latent vector. Specifically, for a given dataset $\D$, we construct the subset for class $c$ as $\{ \bx | \bx \in \mB_c\}$ $\in \mathbb{R}^{\textrm{b} \times \textrm{d}_\textrm{x}}$, where ${\mB_c} \subset \mX_c$ and $||\mB_c||= \textrm{b}$ by random sampling. We input the sub-dataset into the $\textrm{IntraSetPool}$, the intra-class encoder, to encode class prototype $\mathbf{v}_c \in \mathbb{R}^{1 \times \textrm{d}_{\mathbf{v}_c}}$ for each class $c=1,...,C$: $\mathbf{v}_c =	\textrm{IntraSetPool} \big( \{ \bx | \bx \in \mB_c\} \big)$. Then we further feed the class-specific set representations $\{ \mathbf{v}_c \}_{c=1}^C$ into the $\textrm{InterSetPool}$, the inter-class encoder, to generate the dataset representation $\mathbf{h}_{e} \in \mathbb{R}^{1 \times \textrm{d}_{\mathbf{h}_{e}}}$: $\mathbf{h}_{e} =	\textrm{InterSetPool} \big( \{ \mathbf{v}_c \}_{c=1}^C \big)$.

%.  Those can be rewritten as  $\mathbf{v}_c =	\textrm{IntraSetPool} \big( \{ \bx | \bx \in \mB_c\} \big)$ and $\mathbf{h}_{e} =	\textrm{InterSetPool} \big( \{ \mathbf{v}_c \}_{c=1}^C \big)$.
%\begin{align}
%    \mathbf{v}^\tau_c =	\textrm{IntraSetPool} \big( \{ \bx | \bx \in \mB^\tau_c\} \big),  \quad    
%    \mathbf{h}^\tau_{e} =	\textrm{InterSetPool} \big( \{ \mathbf{v}^\tau_c \}_{c=1}^C \big)
%\end{align}

Both the set encoders are comprised of two building blocks: Set Attention Block (SAB) and Pooling by Multi-head Attention (PMA)~\citep{lee2019set}, where the former learns the features for each element in the set using self-attention while the latter pools the input features into $k$ representative vectors. Please see Section~\ref{sec:BB} of the Appendix for more details. We set $k=1$ to produce a single vector, and stack $\textrm{SAB}$ twice followed by $\textrm{PMA}$ for both set encoders as follows (See Figure~\ref{fig:model_component} (a)):
\begin{align}
    \mathbf{v}_c = \textrm{IntraSetPool} \big( \{ \bx | \bx \in \mB_c\} \big) = \textrm{PMA}\big(\textrm{SAB}\big(\textrm{SAB}\big( \{ \bx | \bx \in \mB_c\} \big)\big)\big) \\
    \mathbf{h}_{e} = \textrm{InterSetPool} \big( \{ \mathbf{v}_c \}_{c=1}^C \big) = \textrm{PMA}\big(\textrm{SAB}\big(\textrm{SAB}\big(\{ \mathbf{v}_c \}_{c=1}^C\big)\big)\big) 
\end{align}
Then the latent code $\bz \in \mathbb{R}^{1 \times \textrm{d}_\bz}$ can be sampled from a dataset-conditioned Gaussian distribution with diagonal covariance where $\textrm{NN}_{\bm{\mu}}, \textrm{NN}_{\bm{\sigma}}$ are single linear layers:
\begin{align}
	\bz \sim q_{\bm{\phi}} ( \bz|\D ) = \mathcal{N} ( \bm{\mu}, \bm{\sigma}^2 ), \text{where}\; \bm{\mu}, \bm{\sigma} = \textrm{NN}_{\bm{\mu}} (\mathbf{h}_{e} ), \textrm{NN}_{\bm{\sigma}} (\mathbf{h}_{e} ) \label{eq:mu_and_sigma}
	%\bz \sim q_{\bm{\phi}} ( \bz|\D ) = \mathcal{N} ( \bm{\mu}, \bm{\sigma}^2 ) \nonumber
\end{align}

%\input{others/figure_graph_decoder} 

\paragraph{Graph Decoding} To generate a DAG $\mathcal{G}$ describing a neural architecture from the latent code $\bz$, we use a Graph Neural Network(GNN)-based decoder $p_{\bm{\theta}} (\G|\bz)$. While GNN-based decoders have been actively used to generate graph-structured data~\citep{liu2018constrained, liao2019gran, jin2020hierarchical}, they are suboptimal for our goal since they generally target undirected graphs and therefore ignore the \textit{topological order} of DAGs. Thus, we use a \textbf{GNN with asynchronous message passing (GNN-AMP)} which allows message passing to happen only along the $\textit{topological order}$ of the DAGs~\citep{zhang2019d}.
The graph decoder starts from an initial hidden state $\mathbf{h}_{v_0}= \textrm{NN}_{\textrm{init}}(\bz)$, where $\textrm{NN}_{\textrm{init}}$ is an MLP followed by $tanh$. For $i^{th}$ node $v_i$ according to \textit{topological order}, we compute the probability of each operation type $\textrm{o}_{v_i} \in \mathbb{R}^{1 \times n_o}$ over $n_\textrm{o}$ operations, given the current graph state as the last hidden node $\mathbf{h}_{\G} := \mathbf{h}_{v_{i}}$. That is, $\textrm{o}_{v_i} = \textrm{NN}_{\textrm{node}} (\mathbf{h}_{\G})$, where $\textrm{NN}_{\textrm{node}}$ is an MLP followed by \textit{softmax}.
When the predicted $v_i$ type is the end-of-graph, we stop the decoding process and connect all leaf nodes to $v_i$. Otherwise we update hidden state $\mathbf{h}_{v_i}^{(t)}$ at time step $t$ as follows:
\begin{align}
    \mathbf{h}^{(t+1)}_{v_i} = \textrm{UPDATE} ( i, \bm{m}_{v_i}^{(t)} ) \label{eq:update} \text{, where }\;\bm{m}_{v_i}^{(t)} = \sum_{ u \in \mathcal{V}_{v_i}^{in} } \textrm{AGGREGATE} ( \mathbf{h}_u^{(t)} )
\end{align}
\vspace{-0.2in}

The function $\textrm{UPDATE}$ is a gated recurrent unit (GRU)~\citep{Cho14}, $i$ is the order of $v_i$, and $\bm{m}_{v_i}^{(t)}$ is the incoming message to $v_i$. The function $\textrm{AGGREGATE}$ consists of mapping and gating functions with MLPs, where $\mathcal{V}_{v_i}^{in}$ is a set of predecessors with incoming edges to $v_i$.
For all previously processed nodes $\big \{ v_j | j= i-1,..., 1 \big \}$, we decide whether to link an edge from $v_j$ to $v_i$ by sampling the edge based on edge connection probability $e_{\{v_j,v_i\}} = \textrm{NN}_{\textrm{edge}} (\mathbf{h}_j, \mathbf{h}_i )$
% \begin{align}
% e_{\{v_j,v_i\}} = \textrm{NN}_{\textrm{edge}} (\mathbf{h}_j, \mathbf{h}_i )
% \end{align}
, where $\textrm{NN}_{\textrm{edge}}$ is a MLP followed by $sigmoid$. We update $\mathbf{h}_{v_i}$ by Eq.~\eqref{eq:update} whenever a new edge is connected to $v_i$. For meta-test, we select the operation with the max probability for each node and edges with $e_{\{v_j,v_i\}}>0.5$. Fig~\ref{fig:model_component}(b) illustrates the decoder. For more details, please see Section~\ref{sec:graph_decoding}.
%Following ~\citep{zhang2019d}, we consider nodes $\big\{ v_j | j= i-1,..., 1 \big\}$ in the reverse order to reflect information from nodes close to $v_i$ to the root node  when deciding whether edge connection.
%Note that the proposed process guarantees the generation of DAG since directed edge is always created from existing nodes to a new node. %Note that while DVAE~\citep{zhang2019d} tackles simple tasks such as reconstruction of DAGs, we aim a more challenging problem of generating a DAG from a latent embedding of a dataset.
%\textbf{Graph Decoding} To generate neural architectures from the latent code $\bz^\tau$, we construct a GNN-based decoder $p_{\bm{\theta}} (\G^\tau|\bz^\tau)$. Graph neural networks have been actively used to generate graph-structured data such as social networks, proteins and molecules~\citep{liu2018constrained, liao2019gran, jin2020hierarchical}. 
%Graph decoders can generate graphs~
%However, since those decoders are based on the simultaneous message passing among nodes, which ignores \textit{topological order} of DAGs, they are suboptimal for our goal. Therefore, we use a \textbf{GNN-based decoder with asynchronous message passing (GNN-AMP)} which allows message passing to happen only along the $\textit{topological order}$ of the DAGs~\citep{zhang2019d}. Please See the  \textbf{Suppl.~\ref{sec:graph_decoding}} for the details. Note that while DVAE~\citep{zhang2019d} demonstrates their performance on the simple task such as graph-to-graph reconstruction, we aim a more challenging problem of generating a DAG from a latent embedding of a dataset. 

\textbf{Meta-training Strategy for NAS}
\label{sec:optimization}
We meta-learn the model using set-amortized inference, by maximizing the approximated evidence lower bound (ELBO) for each task $\tau$ as follows:
\begin{align}
     \max_{\bm{\phi}, \bm{\theta}} \E_{\bz \sim q_{\bm{\phi}} ( \bz |\D )} \big[ \log p_{\bm{\theta}} \big( \G|\bz \big) \big] - \lambda \cdot L_{KL}^\tau \big[ q_{\bm{\phi}} \big( \bz|\D \big)|| p \big( \bz \big) \big] \label{eq:elbo}
\end{align}
where each dimension of prior $p(\bz)$ factorizes into $\mathcal{N}(0,1)$. $L^\tau_{KL}$ is the KL divergence between two multivariate Gaussian distributions which has a simple closed form~\citep{kingma2013auto} and $\lambda$ is the scalar weighting value. Using the reparameterization trick on $\bz$, we can optimize the above objective by stochastic gradient variational Bayes~\citep{kingma2013auto}. The expectation of the log-likelihood of \eqref{eq:elbo} can be rewritten with negative cross-entropy loss $-L^\tau_{CE}$ for nodes and binary cross-entropy loss $-L^\tau_{BCE}$ for edges, and we slightly modify it using the generated set-dependent graph $\tilde \G$ and the ground truth graph $\G$ as the input as follows:
\begin{align}
    -L^\tau_{\bm{\phi}, \bm{\theta}} \big(\D, \G \big) = 
    \sum_{v_i \in \V} {  \Big\{ -L_{CE}^\tau\big( \tilde o_{v_i}, o_{v_i} \big) + \sum_{v_j \in \V_i} -L_{BCE}^\tau \big( \tilde e_{\{v_j, v_i\}}, e_{\{v_j, v_i\}} \big) \Big\}} 
    \label{eq:7}
\end{align}
We substitute the log-likelihood term of the equation (\ref{eq:elbo}) such as equation (\ref{eq:7}) and take negative to the equation (\ref{eq:elbo}) to convert it to the resultant objective $\mathcal{L}^\tau_{\bm{\phi}, \bm{\theta}} ( \D, {\G} )$ as follows:
\begin{align}
    \min_{\bm{\phi}, \bm{\theta}} \sum_{\tau \sim p (\tau)} \mathcal{L}^\tau_{\bm{\phi}, \bm{\theta}} \big( \D, \G \big) =
    \min_{\bm{\phi}, \bm{\theta}} \sum_{\tau \sim p (\tau)} \Big\{ L^\tau_{\bm{\phi}, \bm{\theta}}\big(\D, \G \big) + \lambda \cdot L_{KL}^\tau \big[ q_{\bm{\phi}} \big( \bz|\D \big) ||p \big( \bz \big) \big] \Big\} \label{eq:objective}
\end{align}
We learn our MetaD2A generator by minimizing the final objective to learn $\bm{\phi}, \bm{\theta}$, which are shared across all tasks. In the meta-test stage, for a unseen dataset $\hat{\D}$, we can obtain set-dependent DAGs $\{\hat{\G}_i\}_{i=1}^{n_s}$, with the meta-trained generator parameterized by $\bm{\phi}^*, \bm{\theta}^*$, by feeding $ \hat{\D}$ as the input. Thus our method can generate neural architecture(s) for the novel dataset via set-level amortized inference.

%\input{others/algorithms.tex}
\vspace{-0.05in}
\subsection{Meta-Performance Predictor}
\label{sec:predictor}
\vspace{-0.05in}
We design a meta-performance predictor $f_\omega$ to select the best architecture from the architectures generated by MetaD2A generator, based on their predicted accuaracies on the target task. Since our predictor should accurately predict the model performance for any datasets unlike the predictors used in task-specific NAS, it also meta-learned. The meta-performance predictor consists of a dataset encoder and a graph encoder, followed by two linear layers with $relu$. For dataset encoding, we use the \textbf{Hierarchical Set Pooling} of Section~\ref{sec:generator} which takes $\mathcal{D}$ as an input, using only the mean $\bm{\mu}$ from Eq.~(\ref{eq:mu_and_sigma}) as an output.
We perform a bi-directional encoding of the given graph following \textbf{GNN-AMP}~\citep{zhang2019d}, where given $\mathcal{G}$, we sequentially perform message passing for nodes from the predecessors following the \textit{topological order} of the DAG $\mathcal{G}$ and then reverse the node orders and perform an additional encoding process (See Figure~\ref{fig:model_component} (c), and Section~\ref{sec:bidir} of the appendix for more details). We concatenate the outputs of both the bi-directional graph encoder and the set encoder, and feed them to two linear layers with $relu$ to predict accuracy. We train the predictor $f_\bm{\omega}$ to minimize the MSE loss between the predicted accuracy and the true accuracy $s_i$ of the model on each task: 
\begin{align}
    \min_{\bm{\phi}, \bm{\theta}} \sum_{\tau \sim p (\tau)} \mathcal{L}^\tau_{\bm{\omega}}(s, \mathcal{D}, \mathcal{G}) =
    \min_{\bm{\phi}, \bm{\theta}} \sum_{\tau \sim p (\tau)} (s-f_{\bm{\omega}}(\mathcal{D}, \mathcal{G}))^2 \label{eq:pp_objective}
\vspace{-0.1in}
\end{align}
In the meta-test, the predictor $f_{\bm{\omega}^*} (\hat{s}_i | \hat{\D}, \hat{\G}_i)$ predicts accuracies $\{ \hat{s}_i \}_{i=1}^{n_s}$ for a given $\hat{\D}$ and $\{ \hat{\G_i} \}_{i=1}^{n_s}$ and then select the neural architecture having the highest predicted accuracy among $\{ \hat{s_i} \}_{i=1}^{n_s}$.
% We select the final architecture based on the predicted accuracies of the sampled architectures. The performance predictor $f_{\bm{\omega}}(s|\mathcal{D}, \mathcal{G})$ parameterized by $\bm{\omega}$ is also trained from the task distribution $p(\tau)$ and then select the best performing architecture $\hat{\G}^*$ from $\{ \hat{\G_i} \}_{i=1}^{n_s}$ based on predicted accuracy $\{ \hat{s_i} \}_{i=1}^{n_s}$ in the test.

To our knowledge, the performance predictors proposed in the existing NAS works need re-training for the new dataset since they have no module to handle multiple datasets but only encoders for graphs. On the other hand, our proposed meta-performance predictor consists of a \textbf{dataset encoder} and \textbf{graph encoder} to address such a problem with one training. Moreover, the proposed meta-performance predictor learns meta-knowledge accumulated from multiple tasks of MetaImageNet. Thus, the meta-learned predictor can predict performance for the new unseen dataset without training. As the number of target datasets increases, the time complexity of other predictors linearly increases while ours needs a constant time complexity of O(1). %In addition, none of the existing works in both NAS or meta-learning can handle the scale of meta-learning as our MetaD2A does.
%(training over 1,679 datasets, each of which contains 400 samples) 

%~\input{others/figure_graph_encoder}
\vspace{-0.05in}
\subsection{Comparision with Conventional Meta-NAS}
\label{sec:comp_metanas}
\vspace{-0.05in}
Existing meta-NAS approaches~\citep{elsken2020meta, lian2019towards, shaw2019meta} mainly target few-shot classification and cannot scale to such a large task with a large number of samples, since they rely on gradient-based meta-learning with rollout gradient steps. 
For few-shot learning, taking a few gradient steps is more than enough since there are only a few samples from which we can compute the gradients, but for large-scale learning, taking few gradient steps with minibatch sampling will only consider a very small portion of the samples in the task, which will be largely insufficient for the model to converge. 
Thus the model needs to take a large number of gradient steps with a large number of samples, however, this is extremely costly and almost infeasible when computing second-order derivatives as in MAML.
On the contrary, MetaD2A can handle the large-way many-shot problem tackled by general classification tasks, since it does not require any rollout gradient steps when inferring the architecture. 
For conventional few-shot settings (5-way 5-shot), the number of samples per task is 25. Contrarily, the number of samples of CIFAR-100 used in MetaD2A is $100\times{20}=2,000$ which is $80$ times larger. Further, the number of instances(e.g. 20) can be set to a much larger number. 
Overcoming such a limitation of conventional meta-NAS methods, and meta-learning in general, is one of the main contributions of this work, which is highly novel, in both the perspective of NAS and meta-learning. Further, to compare MetaD2A with meta-NAS methods, we perform experiments on few-shot tasks in the Section~\ref{sec:quali_suppl} of the Appendix.

% Recent NAS methods with gradient-based meta-learning~\citep{elsken2020meta, lian2019towards, shaw2019meta} have shown promising results on adapting to different tasks. However, they are only applicable on small scale tasks such as few-shot classification tasks~\citep{elsken2020meta, lian2019towards} and require high-computation time, due to the multiple unrolling gradient steps for one meta-update of each task. While some attempt to bypass the bottleneck with a first-order approximation~\citep{lian2019towards, shaw2019meta} or parallel computations with GPUs~\citep{shaw2019meta}, but their scalability is intrinsically limited due to gradient updates over a large number of tasks. To tackle such a scalability issue, we perform amortized inference over the multiple tasks by encoding a dataset as the low-dimensional latent vector and exploit fast GNN propagation instead of the expensive gradient update.

